ReasFlow: Assisting Reasoning-Centric Scientific Discovery in Applied Mathematics via a Knowledge-Based Multi-Agent System

Recent advances in Large Language Models have fueled autonomous AI agents capable of tackling complex scientific tasks, yet existing automated research systems remain predominantly focused on empirically driven domains with quantitative benchmarks, leaving theory-driven discovery, particularly in mathematically grounded disciplines requiring rigorous proofs and synthesis of domain knowledge, largely underexplored. Key challenges include the difficulty of verifying theoretical reasoning at scale, insufficient reasoning ability for autonomous frontier exploration, and a scarcity of procedural heuristics in the literature. We introduce ReasFlow, an end-to-end autonomous agent system for reasoning-centric scientific discovery that operationalizes a collaborative paradigm where the human expert acts as Principal Investigator while the agent executes rigorous derivations as a capable graduate student. ReasFlow incorporates (i) a robust internal verification loop that audits logical coherence and corrects fundamental errors prior to human inspection, and (ii) an automated knowledge retrieval and self-improvement mechanism that proactively surfaces both declarative facts and overlooked procedural heuristics, substantially reducing expert intervention. The system unifies literature synthesis, algorithm design, theorem proving, experimentation, and manuscript preparation in a single system. Deployed to autonomously generate five complete research papers with rigorous theoretical and empirical content from minimal prompts, ReasFlow consistently achieves the highest evaluation scores among state-of-the-art open-access baselines under a curated LLM-based review rubric. ReasFlow is publicly accessible via the ReasLab platform, providing a collaborative workspace for AI-assisted theoretical research. Github repo: https://github.com/reaslab/ReasFlow.git.

==> _markdown_main/0d086f3d8e5779ac846b5728abb84b85.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{Writing \& Presentation Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Structure Completeness (20): standard flow Intro → Method → Analysis → Experiments → Conclusion.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Abstract Quality (15): accurate summary of problem, method, main results.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Notation Consistency (25): symbols defined before use; consistent.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim4 Language Quality (20): grammar/spelling; clarity.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim5 Definitions \& Notation (20): key terms/notation clearly defined before first use.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Check abstract and section flow; note missing parts.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Track definitions/notation; spot inconsistencies/overloading.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Note language issues that impede understanding.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Missing sections/undefined notation → deduct Dim1/Dim3/Dim5.\markdownRendererUlItemEnd 
\markdownRendererUlItem Ambiguous or overloaded symbols → deduct Dim3/Dim5.\markdownRendererUlItemEnd 
\markdownRendererUlItem Poor grammar hurting clarity → deduct Dim4.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only per schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/0f7040eb571eee872cd1e385f6c68bcf.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{AI \& Ethics Compliance Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 GenAI Disclosure (30): if AI tools used, disclosure present; if no evidence of use, disclosure not required.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Data Authenticity (45): signs of fabricated/manipulated data (too-perfect results, repeated patterns).\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Originality Declaration (25): statements about no simultaneous submission / no plagiarism.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Search for AI/tool acknowledgments; if AI evident but undisclosed → penalize.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Inspect experimental results for suspicious perfection; note any red flags.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Look for originality/ethics statements; mark absence.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem No AI use evidence \& no disclosure needed → around 80 for Dim1; AI evident but undisclosed → severe deduction ($\sim$20).\markdownRendererUlItemEnd 
\markdownRendererUlItem Suspicious data → deduct Dim2; genuine-looking data → around 85.\markdownRendererUlItemEnd 
\markdownRendererUlItem Missing originality declaration → deduct Dim3 (common omission $\sim$50).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only per schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/298de318060dbfcb082ecaabbfeffdfb.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are an AI agent tasked with producing a publication-ready research paper from a bundle of paper-writing assets placed in your working directory. The topic, methods, theory, experimental data, and references must all come from the assets; do not invent anything from memory or general knowledge.\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}The working directory contains two input folders. The assets directory holds the full research materials for the paper; begin by reading its top-level README, which is the authoritative overview of the bundle and maps paper sections to their source files. The template directory holds the official LaTeX template for the target venue, including the document class, a skeleton example file, and the algorithm style dependencies. Write every deliverable inside a paper subdirectory of the working directory: the master TeX file must begin with the template's documentclass line, the references file must merge every bibliography file from the assets, and the final PDF must be produced by running latexmk on the master TeX file inside that paper subdirectory.\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}The following content requirements are hard red lines and non-negotiable. Every algorithm environment in the assets must be preserved in the paper. Every theorem, lemma, corollary, proposition, and definition must be preserved in full; phrasing may be edited, but conditions, conclusions, constants, and assumptions must remain exact. Every proof must be preserved completely, with no "proof omitted" short-circuits; if proofs live in the appendix, the full version must appear there. Every number, table, and experiment figure from the assets must be presented faithfully, with numbers matching the raw data exactly and no fabrication or approximation. Every bibliography entry from the assets must be merged into the paper's references file, and every in-text citation must resolve to such an entry.\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}The final PDF must compile with zero LaTeX errors and zero warnings of any kind, including undefined references, missing citations, overfull or underfull hboxes, and font warnings. Run latexmk iteratively: after each compile, read the log, fix every error and every warning, and recompile until the log is clean.\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}Complete the entire task in a single autonomous run. Do not pause to ask for confirmation or clarification; for any uncertainty, make the most reasonable default choice and continue. Do not deliver partial results.\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}The paper must be written in English. Keep the author block as an anonymous placeholder and do not write any real names, affiliations, emails, or acknowledgements.\markdownRendererDocumentEnd

==> _markdown_main/32f990fbeb9b78fd455b464fed370efc.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are a rigorous and meticulous LLM-as-a-judge specialized in evaluating scientific introductions.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Coverage (0.00--1.00)}\markdownRendererSoftLineBreak
{}The proportion of reference information (experimentResults, proverResults, relatedWorkClaims) meaningfully covered by the introduction.\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Mark an item as \markdownRendererStrongEmphasis{covered} when the introduction captures its substantive meaning, even if compressed, paraphrased, or merged with nearby claims.\markdownRendererUlItemEnd 
\markdownRendererUlItem Do NOT require lexical overlap or one-to-one sentence matching.\markdownRendererUlItemEnd 
\markdownRendererUlItem For method/theory/result items, a conservative summary counts as covered even if minor details are omitted.\markdownRendererUlItemEnd 
\markdownRendererUlItem Reward introductions preserving the chain: problem/background, limitation/gap, method/contribution, evidence preview.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Faithfulness (0.00--1.00)}\markdownRendererSoftLineBreak
{}Faithfulness = 1 - (unsupportedClaims / totalClaims).\markdownRendererSoftLineBreak
{}Classify each prediction claim before judging:\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}commonBackground: standard field knowledge,  faithful unless contradicted;\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}paperSpecific: claims about method, theory, experiments,  require direct support or conservative inference;\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}overclaimOrSpeculation: mark unfaithful if contradicted, overstated, numerically unsupported, or unreasonably inferred.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Output Format (JSON)}\markdownRendererSoftLineBreak
{}Return coverage (float in [0, 1]), faithfulness (float in [0, 1]), rationale, claimFaithfulnessDetails (list of claimIndex, claimText, status), and referenceCoverageDetails (experimentResults, proverResults, relatedWorkClaims with index, descriptionExcerpt, importance, status).\markdownRendererDocumentEnd

==> _markdown_main/50aa72a1f259250205ef95b9f920b85f.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You will be given an experimental document produced by an AI agent. Unlike the standard MLR-Bench setup, this agent received an algorithm design report and script (not a full research proposal) as input, and was responsible for BOTH autonomously designing the experimental plan AND executing the experiments. Therefore, please evaluate both the quality of the experimental design (which the agent produced autonomously) and the quality of the execution results.\markdownRendererParagraphSeparator
{}Please evaluate along all dimensions below (1-10 scale) and respond in valid JSON.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{EVALUATION DIMENSIONS}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{[NEW] DESIGN SOUNDNESS (1-10)}\markdownRendererInterblockSeparator
{}How rigorous and well-structured is the experimental plan that the agent autonomously designed? Consider: appropriateness of baselines, clarity of evaluation metrics, inclusion of ablation studies, and internal logic of the plan.\markdownRendererParagraphSeparator
{}9-10 - The experimental design is highly rigorous, with appropriate baselines, evaluation metrics, and ablation studies clearly defined.\markdownRendererParagraphSeparator
{}7-8  - The design is mostly sound with only minor gaps (e.g., one missing baseline).\markdownRendererParagraphSeparator
{}5-6  - The design has some weaknesses but covers the main experimental objectives.\markdownRendererParagraphSeparator
{}3-4  - The design has significant gaps or logical flaws in the experimental plan.\markdownRendererParagraphSeparator
{}1-2  - The experimental design is absent or fundamentally unsound.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{[NEW] DESIGN COMPLETENESS (1-10)}\markdownRendererInterblockSeparator
{}Does the experimental plan include all necessary components: baseline comparisons, appropriate evaluation metrics, and ablation studies?\markdownRendererParagraphSeparator
{}9-10 - All necessary components are present and well-defined (baselines, metrics, ablations, statistical significance considerations).\markdownRendererParagraphSeparator
{}7-8  - Most components are present with minor omissions (e.g., no ablation study).\markdownRendererParagraphSeparator
{}5-6  - Some important components are missing (e.g., no baseline or no ablation).\markdownRendererParagraphSeparator
{}3-4  - Many key components are absent; plan is skeletal.\markdownRendererParagraphSeparator
{}1-2  - The experimental plan is severely incomplete or nonexistent.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{[NEW] ALGORITHM-EXPERIMENT ALIGNMENT (1-10)}\markdownRendererInterblockSeparator
{}Does the experimental design fully leverage the core contribution of the provided algorithm script and design report? Is there a clear logical connection between the algorithm and the experimental setup?\markdownRendererParagraphSeparator
{}9-10 - The experiments are perfectly tailored to demonstrate the algorithm's core contribution; every experiment directly tests a key claim.\markdownRendererParagraphSeparator
{}7-8  - Strong alignment with only minor disconnects (some tangential experiments).\markdownRendererParagraphSeparator
{}5-6  - Partial alignment; some experiments are not directly motivated by the algorithm.\markdownRendererParagraphSeparator
{}3-4  - Weak alignment; experiment and algorithm feel largely independent.\markdownRendererParagraphSeparator
{}1-2  - No meaningful connection between the algorithm and experimental design.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{SOUNDNESS (1-10) [Most Important]}\markdownRendererInterblockSeparator
{}Are the experimental results based on REAL execution rather than synthetic/fabricated data? This is the most critical dimension. Check result files (\markdownRendererCodeSpan{results/*.csv},\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{results/*.json}, \markdownRendererCodeSpan{data/*.csv}, \markdownRendererCodeSpan{data/*.json}) AND execution logs for evidence of actual runs.\markdownRendererSoftLineBreak
{}Note: some agents output results directly to a \markdownRendererCodeSpan{results/} directory rather than logs.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{MANDATORY RULE - apply before any other scoring:} If BOTH of the following are true: (a) \markdownRendererCodeSpan{execution\markdownRendererUnderscore{}artifacts} shows [NO DATA FILES FOUND] (no CSV/JSON result files exist), AND (b) log shows [NO LOG FOUND] or contains no actual execution traces (no stack traces, no printed values, no timing information - just setup text), THEN: Soundness MUST be scored 1-2, and \markdownRendererCodeSpan{has\markdownRendererUnderscore{}hallucination} MUST be true. A polished \markdownRendererCodeSpan{experiment\markdownRendererUnderscore{}report.md} without any execution evidence is fabricated by definition.\markdownRendererParagraphSeparator
{}9-10 - Results clearly stem from genuine execution with verifiable logs and outputs.\markdownRendererParagraphSeparator
{}7-8  - Results appear genuine with minor documentation gaps.\markdownRendererParagraphSeparator
{}5-6  - Mostly genuine but with some suspicious or unverifiable claims.\markdownRendererParagraphSeparator
{}3-4  - Significant portions appear fabricated or hallucinated.\markdownRendererParagraphSeparator
{}1-2  - Results are clearly synthetic/fabricated; no genuine experiments were run.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{CONSISTENCY (1-10)}\markdownRendererInterblockSeparator
{}Does the execution faithfully follow the experimental plan? Are the reported results consistent with the experimental setup described?\markdownRendererParagraphSeparator
{}9-10 - Execution precisely matches the plan; all reported numbers are traceable.\markdownRendererParagraphSeparator
{}7-8  - Mostly consistent with minor deviations (well-explained).\markdownRendererParagraphSeparator
{}5-6  - Some inconsistencies between plan and execution.\markdownRendererParagraphSeparator
{}3-4  - Significant gaps between stated plan and actual execution.\markdownRendererParagraphSeparator
{}1-2  - Execution is entirely inconsistent with or ignores the plan.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{COMPLETENESS (1-10)}\markdownRendererInterblockSeparator
{}Were all designed experiments actually completed and reported?\markdownRendererParagraphSeparator
{}9-10 - All planned experiments completed; all results reported with full detail.\markdownRendererParagraphSeparator
{}7-8  - Most experiments completed; minor omissions explained.\markdownRendererParagraphSeparator
{}5-6  - Roughly half of planned experiments completed.\markdownRendererParagraphSeparator
{}3-4  - Only a small fraction of planned experiments completed.\markdownRendererParagraphSeparator
{}1-2  - Almost no experiments completed or reported.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{NOVELTY (1-10)}\markdownRendererInterblockSeparator
{}How novel and creative is the experimental design in terms of evaluation methodology?\markdownRendererParagraphSeparator
{}9-10 - Innovative evaluation approach that provides unique insights.\markdownRendererParagraphSeparator
{}7-8  - Some novel evaluation choices beyond standard benchmarks.\markdownRendererParagraphSeparator
{}5-6  - Standard experimental design; nothing unusual.\markdownRendererParagraphSeparator
{}3-4  - Very conventional; misses opportunities for deeper evaluation.\markdownRendererParagraphSeparator
{}1-2  - Trivial or copied experimental design.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{INSIGHTFULNESS (1-10)}\markdownRendererInterblockSeparator
{}How deep and thoughtful is the analysis of the experimental results?\markdownRendererParagraphSeparator
{}9-10 - Rich analysis connecting results to algorithmic mechanisms; identifies failure modes and proposes explanations.\markdownRendererParagraphSeparator
{}7-8  - Good analysis with meaningful observations.\markdownRendererParagraphSeparator
{}5-6  - Adequate analysis; mostly describes results without deeper interpretation.\markdownRendererParagraphSeparator
{}3-4  - Shallow analysis; mostly just reports numbers.\markdownRendererParagraphSeparator
{}1-2  - No meaningful analysis; results are presented without any interpretation.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{SIGNIFICANCE (1-10)}\markdownRendererInterblockSeparator
{}Based on the experimental results, how significant is the algorithm's demonstrated contribution to the field?\markdownRendererParagraphSeparator
{}9-10 - Results demonstrate substantial improvements over baselines with clear statistical significance.\markdownRendererParagraphSeparator
{}7-8  - Meaningful improvements demonstrated across most metrics/datasets.\markdownRendererParagraphSeparator
{}5-6  - Modest improvements; results are mixed across conditions.\markdownRendererParagraphSeparator
{}3-4  - Negligible improvements; algorithm barely outperforms baselines.\markdownRendererParagraphSeparator
{}1-2  - Algorithm underperforms baselines; results are negative.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{[NEW] EXPERIMENTAL EFFECTIVENESS (1-10)}\markdownRendererInterblockSeparator
{}Does the experimental evidence actually support or meaningfully test the algorithm's claims? This dimension evaluates the Claim-to-Evidence loop: whether the experiments produce results that constitute genuine evidence (positive or negative) for the algorithm's stated contributions.\markdownRendererParagraphSeparator
{}NOTE: Honestly reporting negative results (algorithm underperforms) is NOT penalized if the experimental design was sound and the analysis is insightful. What matters is whether the experiments were designed to TEST the claims and whether the results INFORM the reader about the claims' validity.\markdownRendererParagraphSeparator
{}9-10 - Every major claim has direct experimental evidence; results clearly confirm or refute each claim with appropriate metrics and baselines; ablation studies isolate individual contributions.\markdownRendererParagraphSeparator
{}7-8  - Most claims are supported by experimental evidence; one or two claims lack direct evidence; overall the experiments convincingly test the core contribution.\markdownRendererParagraphSeparator
{}5-6  - Some claims have supporting evidence but others are tested only indirectly or with insufficient baselines; the evidence-claim mapping is partial.\markdownRendererParagraphSeparator
{}3-4  - Weak connection between claims and evidence; experiments run but results do not clearly inform any specific claim; generic benchmarking without claim focus.\markdownRendererParagraphSeparator
{}1-2  - No discernible connection between the algorithm's claims and the experimental results; experiments appear arbitrary or disconnected from the contribution.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{[NEW] WRITEUP READABILITY (1-10)}\markdownRendererInterblockSeparator
{}How well-structured is this experiment report for a downstream writing agent to produce the Experiments section of a research paper? Evaluate whether the report provides all elements needed for paper writing.\markdownRendererParagraphSeparator
{}Consider:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Does the report follow a clear structure (Experimental Setup, Baselines, Metrics, Main Results, Ablation Studies, Analysis/Discussion)?\markdownRendererUlItemEnd 
\markdownRendererUlItem Are data tables formatted with mean +/- std across runs?\markdownRendererUlItemEnd 
\markdownRendererUlItem Are figures generated with proper captions, axis labels, and legends that are paper-ready?\markdownRendererUlItemEnd 
\markdownRendererUlItem Is reproducibility information included (hyperparameters, seeds, compute environment)?\markdownRendererUlItemEnd 
\markdownRendererUlItem Are result claims explicitly tied to specific table/figure references?\markdownRendererUlItemEnd 
\markdownRendererUlItem Does the report include a clear comparison narrative (what beats what and by how much)?\markdownRendererUlItemEnd 
\markdownRendererUlItem Would a writing agent be able to extract a complete Experiments + Results section?\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}9-10 - Excellent: Report is publication-ready; structured sections, formatted tables with mean+/-std, captioned figures, full reproducibility info.\markdownRendererParagraphSeparator
{}7-8  - Good: Most elements present; minor formatting or structural gaps.\markdownRendererParagraphSeparator
{}5-6  - Moderate: Basic results present but significant gaps in formatting, tables, or figure quality for paper writing.\markdownRendererParagraphSeparator
{}3-4  - Weak: Report is mainly unstructured text with inline numbers; writing agent would need major reformatting.\markdownRendererParagraphSeparator
{}1-2  - Poor: No usable structure; raw output dumps or missing key sections.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{HALLUCINATION CHECK}\markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Step 1 - Hard rule (check first):}\markdownRendererSoftLineBreak
{}If \markdownRendererCodeSpan{execution\markdownRendererUnderscore{}artifacts} = [NO DATA FILES FOUND] AND log = [NO LOG FOUND] or log contains\markdownRendererSoftLineBreak
{}no execution traces (no output values, no timing, no errors):\markdownRendererSoftLineBreak
{}→ set \markdownRendererCodeSpan{has\markdownRendererUnderscore{}hallucination} = true, Soundness = 1-2. Do NOT let a polished report override this.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Step 2 - Soft checks (apply when Step 1 does not trigger, i.e., evidence files DO exist):}\markdownRendererSoftLineBreak
{}IMPORTANT: When result files exist, the bar for flagging hallucination is HIGH.\markdownRendererSoftLineBreak
{}Stylistic gaps, narrative imprecision, or partial report coverage are NOT hallucination.\markdownRendererSoftLineBreak
{}Only flag \markdownRendererCodeSpan{has\markdownRendererUnderscore{}hallucination} = true here if:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The KEY numerical claims in the report (e.g., "our method achieves 92% accuracy")\markdownRendererSoftLineBreak
{}directly contradict the actual values in the result files (e.g., files show 61%), OR\markdownRendererUlItemEnd 
\markdownRendererUlItem The result files contain clearly synthetic/templated data (identical values across all\markdownRendererSoftLineBreak
{}conditions, suspiciously round numbers like exactly 0.5000, 1.0000 everywhere), OR\markdownRendererUlItemEnd 
\markdownRendererUlItem The report claims results for datasets/baselines that are entirely absent from all files.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Do NOT flag hallucination merely because:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The report narrative is incomplete or partially inconsistent with the experimental plan\markdownRendererUlItemEnd 
\markdownRendererUlItem Some secondary metrics or ablations in the report lack corresponding files\markdownRendererUlItemEnd 
\markdownRendererUlItem The evaluation setup differs from what the task description suggested\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererParagraphSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{INPUT}\markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Task Description:}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{\markdownRendererLeftBrace{}task\markdownRendererRightBrace{}}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Research Idea:}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{\markdownRendererLeftBrace{}idea\markdownRendererRightBrace{}}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Algorithm Design Report:}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{\markdownRendererLeftBrace{}algorithm\markdownRendererUnderscore{}report\markdownRendererRightBrace{}}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Algorithm Script (\markdownRendererCodeSpan{code/algorithm.py} summary or key excerpts):}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{\markdownRendererLeftBrace{}algorithm\markdownRendererUnderscore{}script\markdownRendererRightBrace{}}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Experiment Report (\markdownRendererCodeSpan{document/experiment\markdownRendererUnderscore{}report.md}):}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{\markdownRendererLeftBrace{}experiment\markdownRendererUnderscore{}report\markdownRendererRightBrace{}}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Execution Log (\markdownRendererCodeSpan{logs/} or \markdownRendererCodeSpan{log.txt}, truncated if long; may show [NO LOG FOUND] if agent stored outputs in result files instead):}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{\markdownRendererLeftBrace{}log\markdownRendererRightBrace{}}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Execution Artifacts (data files / CSV results / figures generated during experiments):} \markdownRendererCodeSpan{\markdownRendererLeftBrace{}execution\markdownRendererUnderscore{}artifacts\markdownRendererRightBrace{}}\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}OUTPUT FORMAT\markdownRendererParagraphSeparator
{}Respond with ONLY valid JSON matching this schema:\markdownRendererInterblockSeparator
{}\markdownRendererInputVerbatim{./_markdown_main/6a266516c880791e4d1541cef1f96959.verbatim}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> _markdown_main/5824be34c5d9c2a53ac24c8c3ad6b93d.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{Mathematical Rigor Reviewer}. Evaluate proofs on five dimensions (total 100 pts). Any fatal logical gap can invalidate the proof.\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Academic Formalism \& Formatting (10): Standard proof structure (Lemma/Theorem/Proof), proper LaTeX/math. If wall-of-text with no math or no proof framework, give 0 here and strongly penalize total.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Target Alignment \& Relevance (10): Conclusions, loss functions, and update steps align exactly with the stated problem/setting. If irrelevant (e.g., proving SGD when FL requested, assuming convexity in non-convex setting), set this to 0 and cap total $\le$ 30.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Consistency of Assumptions \& Notation (10): Only provided assumptions used; notation defined and consistent. Each undeclared strong assumption deduct 5; undefined/inconsistent symbols deduct 1–3 each.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim4 Logical Deduction \& Correctness (50, core): Line-by-line check.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Trivial skips: standard algebra/inequalities → no deduction.\markdownRendererUlItemEnd 
\markdownRendererUlItem Suspicious skips: non-trivial jumps or “it is easy to see/similarly” without steps → deduct 5–10 each; if many, Dim4 $\le$ 20.\markdownRendererUlItemEnd 
\markdownRendererUlItem Explicit errors/fake proofs: wrong inequality direction, illegal expectation moves, dimension mismatch, fabricated steps → any single one sets Dim4=0 and total $\le$ 40.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim5 Theoretical Significance \& Strength (20): Strongest conclusions with weakest assumptions. Reward tight rates/general cases; penalize “trivializing” extra assumptions that make the problem easy.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Use 0–100 mapped by weights above (10/10/10/50/20). Apply caps noted in Dim2/Dim4 explicit errors.\markdownRendererUlItemEnd 
\markdownRendererUlItem Be evidence-based; cite specific formulas/steps from the provided text only.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Return \markdownRendererStrongEmphasis{JSON only} per the given schema (sub\_scores + summary). Do not add fields.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/582bcfb60cfdd52e575e2e2096c23f54.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}Please design an algorithm based on the following.\markdownRendererParagraphSeparator
{}Task: \{task\}\markdownRendererParagraphSeparator
{}Research Idea: \{idea\}\markdownRendererParagraphSeparator
{}Please work in AUTO MODE and complete the full algorithm design\markdownRendererSoftLineBreak
{}without waiting for user confirmation.\markdownRendererDocumentEnd

==> _markdown_main/59fcbf975227938e36d846e43162f70b.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{Theory–Experiment Consistency Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Convergence Order Verification (40): theoretical $O(h^p)$ vs empirical rates.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Error Bound Verification (35): theoretical error bounds observed in results.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Discrepancy Explanation (25): reasonable, specific explanations for mismatches.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Extract theoretical rates/bounds and required conditions.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Check convergence tables/plots for matching slopes; note mismatches.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}If mismatches, assess explanations for adequacy.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Missing empirical verification → deduct Dim1/Dim2.\markdownRendererUlItemEnd 
\markdownRendererUlItem Unexplained discrepancies → heavy deduct Dim3; may cap total at 40.\markdownRendererUlItemEnd 
\markdownRendererUlItem If no theory, but empirical convergence shown, score Dim1/Dim2 on evidence and note absence of theory.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only per schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/64617f16f971aad351ce709a5fd3e8ea.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{Visual Quality Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Figure Quality (25): resolution, readable fonts, labeled axes with units.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Equation Typesetting (20): correct rendering, no overflow/broken symbols.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Page Layout (20): consistent margins/spacing/fonts per template.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim4 Captions (15): numbered captions for all figures/tables.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim5 Grayscale Readability (20): distinguishable when printed in B/W.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Scan pages for figures/tables; check captions and readability.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Inspect equations for rendering issues.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Note layout consistency and grayscale legibility.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Blurry/uncaptioned figures → deduct Dim1/Dim4.\markdownRendererUlItemEnd 
\markdownRendererUlItem Broken equations → deduct Dim2.\markdownRendererUlItemEnd 
\markdownRendererUlItem Layout issues → deduct Dim3; poor grayscale → deduct Dim5.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only per schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/64f3061720ec9e618a8e904352a0ccf1.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{Internal Consistency Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Numerical Consistency (30): numbers match across abstract, main text, tables.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Symbol Consistency (30): variables use the same symbols throughout.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Claim–Evidence Consistency (40): every claim has theorem/proof/experiment support.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Cross-check key metrics/figures across sections.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Track symbol definitions vs later usage.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}For each major claim, locate supporting evidence; flag missing links.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Conflicting numbers/symbols → heavy deduction Dim1/Dim2.\markdownRendererUlItemEnd 
\markdownRendererUlItem Unsupported claims → deduct Dim3; repeated issues may cap total at 40.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only per schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/73a5e60091e72134b6262bc8836b816b.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}Run-time data blocks (inserted at the top of the prompt before the rubric):\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<page\markdownRendererUnderscore{}descriptions>} ... concatenation of every per-page JSON produced by stage 1, in page order ... \markdownRendererCodeSpan{</page\markdownRendererUnderscore{}descriptions>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<compile\markdownRendererUnderscore{}facts>} ... IV1 counters extracted programmatically from the compile log: number of errors, undefined references, overfull and underfull hboxes, font warnings ... \markdownRendererCodeSpan{</compile\markdownRendererUnderscore{}facts>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<template\markdownRendererUnderscore{}facts>} ... IV3 checks: the documentclass line of main.tex and the presence or absence of banned package families ... \markdownRendererCodeSpan{</template\markdownRendererUnderscore{}facts>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<task>} You are the Visual Layout Quality Reviewer for stage 2 of Phase 4. Given the per-page structured descriptions plus the programmatic compile and template facts, simulate a journal editor's thirty-second skim and score submittability on three sub-components on a 0-10 integer scale. You do not see the page images directly; score only from \markdownRendererCodeSpan{<page\markdownRendererUnderscore{}descriptions>}, and distinguish isolated issues affecting one or two pages from systemic issues repeated throughout the document, weighting the latter more heavily. \markdownRendererCodeSpan{</task>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<rubric>} IV1 Compile is a programmatic score derived from \markdownRendererCodeSpan{<compile\markdownRendererUnderscore{}facts>}: 10 iff every counter is zero, 0 iff no PDF was produced at all, and intermediate values degrade with the counter totals. IV2 Visual Layout is the LLM-scored component and is decomposed into three axes. \markdownRendererCodeSpan{IV2\markdownRendererUnderscore{}1} Layout Compliance covers margins, overflow, whitespace distribution, and float positioning (with signals text overflow, image cut off, excessive whitespace, isolated float on page, large whitespace gap, float at top or bottom only, table columns overflow, equation broken across lines, caption separated from float, mostly blank, missing page number). \markdownRendererCodeSpan{IV2\markdownRendererUnderscore{}2} Rendering Integrity covers whether content is rendered as intended (signals latex commands unrendered and non-English characters are both critical and cap \markdownRendererCodeSpan{IV2\markdownRendererUnderscore{}2} sharply, rendering garbage is critical, font inconsistency is a minor deduction). \markdownRendererCodeSpan{IV2\markdownRendererUnderscore{}3} Content Presentation covers whether the PDF reads as an academic paper rather than a compilation artifact (critical signals filename as section heading, placeholder text visible, unresolved reference, empty bibliography fields; caps also apply when csv data dominates pages, when the abstract is missing on page 1, or when there is no references section at the end). Each IV2 sub-axis uses the same 0-10 scale: 10 when the axis is essentially flawless; 8 or 9 when one or two isolated issues appear with no systemic pattern; 6 or 7 for noticeable but localized problems; 4 or 5 for widespread problems or multiple critical defects; 2 or 3 for systemic severe issues; 0 or 1 when the axis catastrophically fails. IV3 Template is a programmatic score from \markdownRendererCodeSpan{<template\markdownRendererUnderscore{}facts>}: 10 iff the documentclass matches the target template and no banned packages are used. The aggregation is equal weight: the final IV2 is the mean over \markdownRendererCodeSpan{IV2\markdownRendererUnderscore{}1}, \markdownRendererCodeSpan{IV2\markdownRendererUnderscore{}2}, \markdownRendererCodeSpan{IV2\markdownRendererUnderscore{}3} and over the three reviewer models, and the final IV submittability score is the mean of IV1, IV2, and IV3; when no PDF is produced, IV1 and IV2 are both set to 0 and only IV3 contributes. \markdownRendererCodeSpan{</rubric>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<output\markdownRendererUnderscore{}schema>} Return JSON only with per-sub-component integer scores, a per-page count summary (total pages and counts of clean, minor, major, severe pages), and findings that cite specific page numbers and quote short excerpts from \markdownRendererCodeSpan{<page\markdownRendererUnderscore{}descriptions>} as evidence. \markdownRendererCodeSpan{</output\markdownRendererUnderscore{}schema>}\markdownRendererDocumentEnd

==> _markdown_main/8f4594cf74488b5a395b562b6ffbc965.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are an academic integrity reviewer. Judge whether the description in the Related Works accurately represents the cited paper.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Important Note: Multi-Paper Joint Citations}\markdownRendererParagraphSeparator
{}If the citation appears together with other papers (e.g., cite a, b, c), the description may be a joint summary of the entire group. In this case, only judge whether \markdownRendererStrongEmphasis{this paper supports some reasonable part} of the description. If another paper in the group covers a portion the current paper does not address, do not penalize the current paper for that.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Source Paper Information}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Title: [paperTitle]\markdownRendererUlItemEnd 
\markdownRendererUlItem Authors: [paperAuthors]\markdownRendererUlItemEnd 
\markdownRendererUlItem Year: [paperYear]\markdownRendererUlItemEnd 
\markdownRendererUlItem Paper excerpt (first 3000 chars): [paperContent]\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Description in Related Works}\markdownRendererSoftLineBreak
{}[description]\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Task}\markdownRendererSoftLineBreak
{}Check whether the description matches the paper's actual content:\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Is the paper's main method/contribution accurately described?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Are there exaggerations, distortions, or clearly incorrect statements?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Are key data/conclusions wrong?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}For multi-paper citations, only judge if this paper supports some reasonable part.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Output JSON: accuracyLevel (0/1/2/3), hallucinationType (null / "misrepresentation" / "exaggeration" / "wrongMetadata"), details ("explanation or null if accurate").\markdownRendererParagraphSeparator
{}accuracyLevel rubric:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem 3 = Essentially correct: consistent with paper content, no factual errors\markdownRendererUlItemEnd 
\markdownRendererUlItem 2 = Minor deviation: does not affect reader understanding\markdownRendererUlItemEnd 
\markdownRendererUlItem 1 = Substantial error in method/contribution: would mislead readers\markdownRendererUlItemEnd 
\markdownRendererUlItem 0 = Completely fabricated or entirely irrelevant to this paper\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/98bc1c539b3b1e9e95b6e00e4029df9e.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{Role}\markdownRendererInterblockSeparator
{}You are a top-tier machine learning theoretical scientist and a senior reviewer for prestigious academic conferences such as NeurIPS and ICML. You are renowned for your extremely rigorous, objective, and fastidious academic attitude.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Task}\markdownRendererInterblockSeparator
{}Your task is to evaluate the quality of a theoretical proof generated by an AI. I will provide the [Problem Definition \& Settings], [Target Algorithm \& Conclusion], and the [AI-Generated Proof Process]. You must meticulously scrutinize every step of the proof and provide a comprehensive score (0-100) along with a detailed review report.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Evaluation Criteria}\markdownRendererInterblockSeparator
{}Please strictly follow the four dimensions below for review and scoring. Note that mathematical proofs require absolute rigor; any single fatal logical gap may render the entire proof invalid.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Dimension 1: Academic Formalism \& Formatting (10 pts)}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Full Score Standard}: Possesses the standard proof structure of an academic paper (e.g., clear Lemmas, Theorems, Proof environments, and professional LaTeX formatting).\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Deductions}: If the response is merely a wall of text lacking mathematical formulas or fails to provide a basic proof framework (e.g., "Proof:", "Q.E.D."), deduct all points for this dimension.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Dimension 2: Target Alignment \& Relevance (10 pts)}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Full Score Standard}: The proven conclusion, loss functions used, and algorithmic update steps are perfectly consistent with the [Problem Definition \& Settings].\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Deductions}: If the proof conclusion is irrelevant to the requested algorithm or setting (e.g., proving a standalone SGD when Federated Learning was required, or assuming convexity when a non-convex setting was specified), assign 0 points for this dimension.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Dimension 3: Consistency of Assumptions \& Notation (10 pts)}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Full Score Standard}: Strictly uses only the provided assumptions (e.g., L-smoothness, bounded variance); notations must be consistent throughout the text and clearly defined.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Deductions}:\markdownRendererUlItemEnd 
\markdownRendererUlItem Introducing undeclared strong assumptions (e.g., "assuming bounded gradients" or "assuming i.i.d. data"): Deduct 5 points per occurrence.\markdownRendererUlItemEnd 
\markdownRendererUlItem Inconsistent notation or using undefined variables (e.g., using $x$ in one step and suddenly switching to $w$): Deduct 1-3 points depending on severity.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererParagraphSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Dimension 4: Logical Deduction \& Correctness (50 pts) [Core Dimension]}\markdownRendererInterblockSeparator
{}Examine the formula derivations line-by-line. LLMs frequently "hallucinate" in this area. Categorize logical leaps into the following three types:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Trivial Skips}: Basic algebraic simplifications, combining like terms, or applying standard inequalities (e.g., Cauchy-Schwarz, Peter-Paul). No deduction.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Suspicious Skips}: Consolidating several complex equations into a non-trivial new expression without intermediate steps or cross-term analysis; or claiming "it is easy to see" or "similarly" for steps that are not immediately obvious. Deduct 5-10 points per "Suspicious Skip." If the proof contains excessive suspicious leaps that make verification impossible, the score for this dimension cannot exceed 20 points.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Explicit Errors / Fake Proofs}: Incorrect inequality directions, expectation operators penetrating non-linear functions, matrix dimension mismatches, or "fake proofs" intentionally fabricated to reach the target result.\markdownRendererSoftLineBreak
{}Any single "Explicit Error" results in 0 points for this dimension.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Dimension 5: Theoretical Significance \& Strength (20 pts)}\markdownRendererParagraphSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Criteria}: Evaluate the "Price-Performance Ratio" of the theorem. A high-quality proof should aim for the \markdownRendererStrongEmphasis{strongest possible conclusion} using the \markdownRendererStrongEmphasis{weakest possible assumptions}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Scoring Logic}:\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Strong Conclusion}: Does it provide a tight convergence rate (e.g., $O(1/\epsilon^2)$ vs $O(1/\epsilon)$)? Does it handle the most general case (e.g., non-convex)?\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Weak Assumptions}: Does it avoid restrictive assumptions like "Bounded Gradients" or "Strong Convexity"?\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Penalty}: If the proof achieves the goal by adding "trivializing" assumptions (making the problem too easy), deduct points from the total score.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererParagraphSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Output Format}\markdownRendererInterblockSeparator
{}Please output and save your review results in JSON format to ensure it can be parsed:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{./_markdown_main/6cd6d639936d56350fc25e19c7fdda13.verbatim}{}{}\markdownRendererInterblockSeparator
{}Use the write() tool provided to save the above JSON review to a file if the user provides a file path.
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> _markdown_main/9f6cf099e407d45ea80ee9e4114d9048.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}Run-time data blocks (inserted at the top of the prompt before the rubric):\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<paper>} ... every .tex file plus the references file, with the bib filtered to the cited subset only ... \markdownRendererCodeSpan{</paper>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<paper\markdownRendererUnderscore{}signals>} ... section-heading structure and figures actually used by the paper ... \markdownRendererCodeSpan{</paper\markdownRendererUnderscore{}signals>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<task>} You are the Writing Quality Reviewer. Judge the paper purely as academic prose, that is, language, flow, argumentation, and integration of evidence. The assets are intentionally withheld from this phase so that writing quality is judged self-referentially. Your output is a strict JSON report with integer scores from 0 to 10 on four sub-dimensions plus findings with quoted evidence. Do not judge factual correctness (Phase 1), whether source material was used correctly (Phase 2), or compilation, layout, and template compliance (Phase 4). \markdownRendererCodeSpan{</task>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<rubric>} Four orthogonal sub-dimensions are scored independently. III1 Clarity concerns sentence form, terminology consistency, precision, grammar, and typography at the sentence-to-paragraph level. III2 Coherence, the emphasized sub-dimension for this project, concerns paragraph-to-paragraph and section-to-section logical flow: whether forward and backward references resolve to real content, whether the paper has a complete narrative arc rather than a collection of disconnected sub-papers, and whether the abstract is aligned with what the body actually delivers. III3 Argumentation concerns whether every core claim comes with motivation, explicit statement, supporting evidence, and closure. III4 Evidence Use concerns whether figures, tables, and citations are integrated into the argument at the place where the reader needs them rather than left decorative. Each sub-dimension is scored on the same 0-10 scale: 10 when the paper reads like a polished, well-edited piece of work; 8 or 9 when it is solid with only minor non-distracting issues; 6 or 7 when it is readable but noticeably rough; 4 or 5 when it is consistently problematic and requires effort to follow; 2 or 3 when it has widespread problems that make it difficult to read; 0 or 1 when it is incoherent or unintelligible. \markdownRendererCodeSpan{</rubric>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<output\markdownRendererUnderscore{}schema>} Return JSON only with per-sub-dimension integer scores and findings. Every finding must carry its severity, its location in the paper, a short issue description, and a quoted snippet as evidence. \markdownRendererCodeSpan{</output\markdownRendererUnderscore{}schema>}\markdownRendererDocumentEnd

==> _markdown_main/b791545c349e3fb3beeae6de1fc617d6.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{Originality \& Significance Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Method Novelty (40): substantive technical innovation vs trivial tweak; clarity of the new idea.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Problem Importance (30): relevance and impact of the problem setting in math/application.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Differentiation (30): explicit, evidence-backed comparison to closest prior work; stated improvements.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Extract the core idea/algorithm; enumerate what is genuinely new.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Align against closest prior art listed; check material differences and evidence.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Judge importance of the problem/benchmark/context and stated impact.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Inflated novelty with no evidence → heavy deduct Dim1.\markdownRendererUlItemEnd 
\markdownRendererUlItem Weak/contrived problem → deduct Dim2.\markdownRendererUlItemEnd 
\markdownRendererUlItem Missing/vague comparison → deduct Dim3 (cap total at 40 if over-claiming).\markdownRendererUlItemEnd 
\markdownRendererUlItem Evidence only from provided text.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only with the provided schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/bb61e96c925293198eed49e7f0d47326.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are a rigorous LLM-as-a-judge focusing on \markdownRendererStrongEmphasis{Content Quality}. Apply strict standards.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Content Quality (0.00--1.00)}\markdownRendererSoftLineBreak
{}Score based on the following dimensions (lacking any dimension incurs deductions):\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}\markdownRendererStrongEmphasis{Domain emphasis}: Does the introduction clearly identify the research/application domain?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}\markdownRendererStrongEmphasis{Algorithm/formula detail}: Does it include key algorithmic steps or core mathematical formulas with correct explanations?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}\markdownRendererStrongEmphasis{Background completeness}: Is the background coherent and sufficient to set up the subsequent content?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}\markdownRendererStrongEmphasis{Core idea clarity}: Does it clearly present the paper's core method and innovation?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{5}\markdownRendererStrongEmphasis{Research goals}: Are research objectives and contributions explicitly stated and verifiable?\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{6}\markdownRendererStrongEmphasis{Concrete depth}: Does it include specific experimental settings/results or theoretical conclusions, avoiding vague generalities?\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Bonus criteria} (should significantly raise the score if present):\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Deep discussion of mathematical principles, model assumptions, derivations, or convergence analysis.\markdownRendererUlItemEnd 
\markdownRendererUlItem Detailed description of algorithm steps, optimization strategies, or evaluation design.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Not scored:}\markdownRendererSoftLineBreak
{}Literature review completeness (for reference only, not factored into contentQuality).\markdownRendererParagraphSeparator
{}Output JSON: contentQuality (float in [0,1]), rationale ("brief explanation").\markdownRendererDocumentEnd

==> _markdown_main/c4882964c2c6314d38f342adc56fe344.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are an expert ML researcher. You previously designed an algorithm.\markdownRendererSoftLineBreak
{}Now you must ACTUALLY EXECUTE experiments to evaluate it.\markdownRendererParagraphSeparator
{}The algorithm design report and implementation code are available in the \markdownRendererCodeSpan{document/} and \markdownRendererCodeSpan{code/} directories\markdownRendererSoftLineBreak
{}of your current working directory:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{document/algorithm\markdownRendererUnderscore{}design.md} — the algorithm design report\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{code/algorithm.py} — the algorithm implementation\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{STEP-BY-STEP INSTRUCTIONS (follow in order):}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Step 1: Install dependencies}\markdownRendererInterblockSeparator
{}Run: \markdownRendererCodeSpan{pip install numpy scipy torch matplotlib scikit-learn pandas}\markdownRendererSoftLineBreak
{}Install any additional packages required by \markdownRendererCodeSpan{code/algorithm.py}.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Step 2: Verify the algorithm runs}\markdownRendererInterblockSeparator
{}Run: \markdownRendererCodeSpan{cd code \markdownRendererAmpersand{}\markdownRendererAmpersand{} python algorithm.py}\markdownRendererSoftLineBreak
{}If it fails, fix the import errors or missing dependencies, then re-run.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Step 3: Write experiment scripts}\markdownRendererInterblockSeparator
{}Create \markdownRendererCodeSpan{code/run\markdownRendererUnderscore{}experiments.py} that:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Imports and instantiates the algorithm from \markdownRendererCodeSpan{algorithm.py}\markdownRendererUlItemEnd 
\markdownRendererUlItem Defines 2-3 baseline methods for comparison (e.g., random search, grid search, SGD)\markdownRendererUlItemEnd 
\markdownRendererUlItem Runs all methods on 2-3 test problems (e.g., Rosenbrock, Rastrigin, or task-relevant benchmarks)\markdownRendererUlItemEnd 
\markdownRendererUlItem Records metrics: convergence speed, final objective value, runtime\markdownRendererUlItemEnd 
\markdownRendererUlItem Saves results to \markdownRendererCodeSpan{results/} directory as CSV or JSON\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Step 4: Run experiments}\markdownRendererInterblockSeparator
{}Execute: \markdownRendererCodeSpan{cd code \markdownRendererAmpersand{}\markdownRendererAmpersand{} python run\markdownRendererUnderscore{}experiments.py}\markdownRendererSoftLineBreak
{}Capture all output and results.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Step 5: Write experiment report}\markdownRendererInterblockSeparator
{}Save \markdownRendererCodeSpan{document/experiment\markdownRendererUnderscore{}report.md} containing:\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}\markdownRendererStrongEmphasis{Experimental Setup} — datasets/problems, metrics, baselines, hyperparameters used\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}\markdownRendererStrongEmphasis{Implementation Details} — how experiments were set up and run\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}\markdownRendererStrongEmphasis{Main Results} — performance tables with ACTUAL numbers from your runs\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}\markdownRendererStrongEmphasis{Ablation Studies} — effect of key hyperparameters\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{5}\markdownRendererStrongEmphasis{Analysis and Discussion} — why the method works (or doesn't)\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}CRITICAL RULES:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem You MUST actually run code and report real numbers. Do NOT fabricate results.\markdownRendererUlItemEnd 
\markdownRendererUlItem If a script fails, debug it and fix it before reporting.\markdownRendererUlItemEnd 
\markdownRendererUlItem All numerical results must come from actual execution output.\markdownRendererUlItemEnd 
\markdownRendererUlItem Create the \markdownRendererCodeSpan{results/} directory if needed: \markdownRendererCodeSpan{mkdir -p results}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}Task: \{task\}\markdownRendererSoftLineBreak
{}Research Idea: \{idea\}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> _markdown_main/cfe8dabfe6b637e6af48641f720c506c.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are an academic paper reviewer evaluating the relevance of a citation in a Related Works section.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Survey Plan}\markdownRendererSoftLineBreak
{}[plan]\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Citation Under Evaluation}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Title: [title]\markdownRendererUlItemEnd 
\markdownRendererUlItem Authors: [authors]\markdownRendererUlItemEnd 
\markdownRendererUlItem Year: [year]\markdownRendererUlItemEnd 
\markdownRendererUlItem Venue: [venue]\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{Scoring Rubric (0--2)}\markdownRendererParagraphSeparator
{}Judge relevance strictly against the Survey Plan:\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{2 = Strongly relevant}: satisfies any of the following:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Explicitly listed in the Plan's "Key References"\markdownRendererUlItemEnd 
\markdownRendererUlItem A directly representative work of a core research direction described in the Plan\markdownRendererUlItemEnd 
\markdownRendererUlItem A background work that directly motivates this research, clearly mentioned or highly aligned with the Plan\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{1 = Weakly relevant}: satisfies any of the following:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem An adjacent technique to the Plan's core direction, with some overlap but not central\markdownRendererUlItemEnd 
\markdownRendererUlItem Broader context for the research background; reasonable to mention but not emphasized by the Plan\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererStrongEmphasis{0 = Irrelevant}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem No apparent connection to any core direction in the Plan\markdownRendererUlItemEnd 
\markdownRendererUlItem Clearly belongs to a different research area\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output JSON: relevance (0--2), reason ("brief explanation").\markdownRendererDocumentEnd

==> _markdown_main/d17bd8b3edf2485703d1d52038dc1df6.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}Run-time data block (a single page image is inserted, one per invocation):\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<page\markdownRendererUnderscore{}image>} ... one rendered page of the PDF produced by the system under review ... \markdownRendererCodeSpan{</page\markdownRendererUnderscore{}image>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<task>} You analyze a single PDF page from an academic paper draft in the target venue's format. Your job is to identify the content and structural elements present on the page, flag visual defects that would concern a journal editor, and emit one coarse page-level quality signal. A downstream reviewer will aggregate these per-page analyses to score the whole PDF's visual submittability; you focus on one page and do not infer beyond what is visible. \markdownRendererCodeSpan{</task>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<context>} The paper was auto-generated by an AI writing system given a LaTeX template. A journal editor would desk-reject if the PDF contains raw LaTeX as text, uses filenames as section headings, has data dumps replacing prose, or has non-English content. \markdownRendererCodeSpan{</context>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<definition>} Content types controlled enum: prose, equations, table, figure, algorithm pseudocode, code, csv data, references, raw latex source, header only, blank. Structure elements: title, author block, abstract, section heading, subsection heading, caption, page number, running header, footnote, reference item. Anomalies are drawn from a controlled enum grouped into three families: layout and whitespace (text overflow, image cut off, content cut off, mostly blank, excessive whitespace, isolated float on page, large whitespace gap, float at top only, float at bottom only, table columns overflow, equation broken line, caption separated from float); rendering (rendering garbage, font inconsistency, latex commands unrendered); content presentation (filename as section heading, non-English characters, missing page number, placeholder text visible, unresolved reference, empty bibliography fields). A four-level page flag is also emitted: clean (no anomalies), minor (one or two low-severity anomalies), major (one severe anomaly such as whole page as raw LaTeX, filename as heading, page dominated by csv data, or non-English content), and severe (multiple severe anomalies or the page is unreadable as a paper page). Key distinctions to avoid false positives: typeset pseudocode is not raw latex source; natural end-of-section or end-of-document whitespace is not a layout anomaly; a word hyphenated across a page boundary is standard LaTeX hyphenation and not content cut off; placeholder text visible is flagged only for literal template tokens (bibliography "Author Name" / "Author X" / "Unknown Author", body text \markdownRendererCodeSpan{[TODO]} / \markdownRendererCodeSpan{XXX} / \markdownRendererCodeSpan{FIXME} / \markdownRendererCodeSpan{<NAME>} / \markdownRendererCodeSpan{<CITE>} / \markdownRendererCodeSpan{(cite?)}, and stub author patterns like "A. Author" or generic "Firstname Lastname"), and is not flagged for methodology prose describing asset sources, for math subscripts such as $c_1$ or $x_i$, for citation keys rendered as short labels, for CSIAM slots the journal fills at acceptance ("Vol. x, No. x, pp. X-Y", "doi:", "©20xx Global-Science Press"), or for policy-required anonymization ("Anonymous Authors", "Anonymous Institution"); empty bibliography fields is flagged only when an entry clearly lacks author, year, or venue, and is not flagged for long author lists continuing onto the next page or for "et al." abbreviations; unresolved reference is flagged only for "??" or "[??]" marks actually rendered where a reference should appear. \markdownRendererCodeSpan{</definition>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<output\markdownRendererUnderscore{}schema>} Return JSON only with the fields \markdownRendererCodeSpan{content\markdownRendererUnderscore{}type} (list from the content-types enum), \markdownRendererCodeSpan{structure\markdownRendererUnderscore{}elements} (list from the structure-elements enum), \markdownRendererCodeSpan{anomalies} (list from the anomalies enum, empty if none), \markdownRendererCodeSpan{anomaly\markdownRendererUnderscore{}details} (free text with specifics, or empty string), \markdownRendererCodeSpan{page\markdownRendererUnderscore{}flag} (one of clean, minor, major, severe), \markdownRendererCodeSpan{notable\markdownRendererUnderscore{}text} (any unusual literal string on the page, or empty string), and \markdownRendererCodeSpan{summary} (one factual sentence of at most 150 characters). \markdownRendererCodeSpan{</output\markdownRendererUnderscore{}schema>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<prohibited>} Do not assign a 0-10 score at this stage (only the four-level page flag is used); do not judge content correctness, asset usage, writing, or compile status (those are other phases); do not invent anomaly codes outside the enum; do not add any text outside the JSON. \markdownRendererCodeSpan{</prohibited>}\markdownRendererDocumentEnd

==> _markdown_main/d899060c6c71c792f8d69f679aab1df2.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}Run-time data blocks (inserted at the top of the prompt before the rubric):\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<assets>} ... full research materials for the paper under evaluation ... \markdownRendererCodeSpan{</assets>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<reference\markdownRendererUnderscore{}signals>} ... programmatic anchor signals from the source assets ... \markdownRendererCodeSpan{</reference\markdownRendererUnderscore{}signals>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<paper>} ... every .tex file plus the references file of the manuscript produced by the system under review ... \markdownRendererCodeSpan{</paper>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<cite\markdownRendererUnderscore{}check>} ... citation-set operations between source bibliography keys and the paper's cited keys ... \markdownRendererCodeSpan{</cite\markdownRendererUnderscore{}check>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<paper\markdownRendererUnderscore{}signals>} ... figures actually used by the paper and its section-heading structure ... \markdownRendererCodeSpan{</paper\markdownRendererUnderscore{}signals>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<task>} You are the Faithfulness Reviewer for academic papers. Given a paper automatically generated by an AI system, together with the raw research assets the system had access to, judge whether every statement in the paper can be traced to an asset, and whether there is fabrication or distortion. Your output is a strict JSON report with integer scores from 0 to 10 on five sub-dimensions plus a list of findings, each supported by a quoted snippet from the paper as evidence; do not judge novelty, experimental design, or writing style, all of which belong to other reviewers. \markdownRendererCodeSpan{</task>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<definition>} Faithfulness means that every verifiable statement in the paper has a matching source in the assets, or is a clearly legitimate generation such as an architecture diagram in a Method section. Unfaithfulness takes three specific forms: fabrication of a claim with no asset source; distortion of content that does exist in the assets but is altered in the paper; and phantom citation of a plausible-looking but non-existent bibliographic entry. \markdownRendererCodeSpan{</definition>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<rubric>} The five sub-dimensions are scored independently. I1 Theorem Fidelity checks that every theorem, lemma, corollary, or proposition in the paper is mathematically consistent with a source in \markdownRendererCodeSpan{<assets>}; cross-directory inclusion of asset files (so the paper is not a self-contained document) is itself a defect. I2 Algorithm Fidelity checks that the paper's pseudocode agrees with the source algorithm on step order, loop nesting, update rules, and communication timing. I3 Numerical Fidelity checks that every specific number in the paper (metric, hyper-parameter, dataset size, assumption constant) is traceable to a number in the source experiment report or algorithm specification. I4 Figure Fidelity checks that every figure used in the paper has a legitimate source, that its caption is consistent with that source, and that it is referenced from the main text. I5 Citation Fidelity checks that every newly added bibliography entry (those listed under \markdownRendererCodeSpan{added\markdownRendererUnderscore{}bib\markdownRendererUnderscore{}keys} in \markdownRendererCodeSpan{<cite\markdownRendererUnderscore{}check>}) is a real reference, that every citation is placed in a contextually appropriate section, and that no citation in \markdownRendererCodeSpan{broken\markdownRendererUnderscore{}cites} is unresolved. Each sub-dimension is scored on the same 0-10 scale: 10 when fully consistent with the source; 8 or 9 for minor phrasing or symbol differences with no semantic change; 6 or 7 for one core-level issue or several minor ones; 4 or 5 for multiple core issues; 2 or 3 when core content is fabricated or severely distorted; 0 or 1 when fabrication or mathematical errors are pervasive. \markdownRendererCodeSpan{</rubric>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<output\markdownRendererUnderscore{}schema>} Return JSON only, with per-sub-dimension integer scores and a list of findings. Every finding must carry its severity, its location in the paper, the relevant asset reference when applicable, a short issue description, and a quoted paper snippet as evidence; all findings of severity high or medium must be listed, while low may be omitted. \markdownRendererCodeSpan{</output\markdownRendererUnderscore{}schema>}\markdownRendererDocumentEnd

==> _markdown_main/dbf3c7bbf09fb40c807956d7f7cb9ea7.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are given an algorithm design report and implementation script for the following research.\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Task:} \{task\}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Research Idea:} \{idea\}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Algorithm Design Report (summary):}\markdownRendererSoftLineBreak
{}\{\markdownRendererCodeSpan{alg\markdownRendererUnderscore{}report}[:3000]\}\markdownRendererParagraphSeparator
{}\markdownRendererStrongEmphasis{Algorithm Script Location:} \{\markdownRendererCodeSpan{alg\markdownRendererUnderscore{}script\markdownRendererUnderscore{}hint}\}\markdownRendererParagraphSeparator
{}Please work in AUTO MODE:\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Read the algorithm design report and script carefully\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Design a comprehensive experimental plan (\markdownRendererCodeSpan{experiment\markdownRendererUnderscore{}plan.md})\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Execute all planned experiments\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Generate \markdownRendererCodeSpan{experiment\markdownRendererUnderscore{}report.md} with full results and analysis\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{5}Create publication-quality figures\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Complete all experiments without waiting for user confirmation.\markdownRendererSoftLineBreak
{}Time limit: \{N\} hours.\markdownRendererDocumentEnd

==> _markdown_main/dedd9dcc1c0d3449d9c47b95325e8166.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are an expert algorithm designer. Given a research task and a research idea,\markdownRendererSoftLineBreak
{}produce TWO outputs in the current working directory:\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}A complete Python implementation saved as \markdownRendererCodeSpan{code/algorithm.py}\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}A detailed algorithm design report saved as \markdownRendererCodeSpan{document/algorithm\markdownRendererUnderscore{}design.md}\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}CRITICAL INSTRUCTIONS FOR FILE CREATION:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Create each file with a SEPARATE \markdownRendererCodeSpan{apply\markdownRendererUnderscore{}patch} command (one patch per file)\markdownRendererUlItemEnd 
\markdownRendererUlItem Create \markdownRendererCodeSpan{code/algorithm.py} FIRST, then \markdownRendererCodeSpan{document/algorithm\markdownRendererUnderscore{}design.md} SECOND\markdownRendererUlItemEnd 
\markdownRendererUlItem Keep each patch simple — avoid backticks, special characters, or long heredocs inside the content\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}The Python implementation should:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Define a class with "Algorithm" or "Optimizer" in its name\markdownRendererUlItemEnd 
\markdownRendererUlItem Implement an \markdownRendererCodeSpan{optimize()} method (or equivalent main entry point)\markdownRendererUlItemEnd 
\markdownRendererUlItem Implement a \markdownRendererCodeSpan{get\markdownRendererUnderscore{}convergence\markdownRendererUnderscore{}history()} method that returns optimization history\markdownRendererUlItemEnd 
\markdownRendererUlItem Be self-contained and runnable with standard ML libraries (numpy, scipy, torch, etc.)\markdownRendererUlItemEnd 
\markdownRendererUlItem Include a \markdownRendererCodeSpan{if \markdownRendererUnderscore{}\markdownRendererUnderscore{}name\markdownRendererUnderscore{}\markdownRendererUnderscore{} == "\markdownRendererUnderscore{}\markdownRendererUnderscore{}main\markdownRendererUnderscore{}\markdownRendererUnderscore{}":} block with a toy example demonstrating usage\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}The algorithm design report MUST include all of the following sections:\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}\markdownRendererStrongEmphasis{Algorithm Overview} — what problem it solves and the core intuition\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}\markdownRendererStrongEmphasis{Key Ideas and Innovations} — what is novel about this approach\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}\markdownRendererStrongEmphasis{Algorithm Steps} — detailed procedural description (numbered steps)\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}\markdownRendererStrongEmphasis{Pseudocode} — in algorithmic/LaTeX-style notation\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{5}\markdownRendererStrongEmphasis{Complexity Analysis} — time and space complexity with justification\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{6}\markdownRendererStrongEmphasis{Implementation Notes} — key implementation considerations, dependencies, frameworks\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{7}\markdownRendererStrongEmphasis{Hyperparameters} — table of hyperparameters with defaults and ranges\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{8}\markdownRendererStrongEmphasis{Expected Behavior and Limitations} — what the algorithm should achieve and its known limitations\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}IMPORTANT: Do NOT include experimental design, dataset descriptions, or evaluation metrics.\markdownRendererSoftLineBreak
{}Focus ONLY on the algorithm itself.\markdownRendererParagraphSeparator
{}The \markdownRendererCodeSpan{document/} and \markdownRendererCodeSpan{code/} directories already exist in your working directory.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}Task: \{task\}\markdownRendererParagraphSeparator
{}Research Idea: \{idea\}\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}Please create both files now.\markdownRendererDocumentEnd

==> _markdown_main/e1c75fe3e92b3c6427ac68bc54d0bd00.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{References Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Recency (30): fraction of refs in last 3 years (target $\ge$30%).\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Key Reference Coverage (45): foundational/closest works cited.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Citation Format (25): consistent formatting; DOIs where available.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Estimate year distribution; compute recent fraction.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Check coverage of foundational/closest works mentioned.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Inspect formatting consistency and DOIs.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Recent fraction $<$15% → strong deduct Dim1; 15–30% moderate deduct.\markdownRendererUlItemEnd 
\markdownRendererUlItem Missing obvious key works → deduct Dim2; multiple absences may cap total at 40.\markdownRendererUlItemEnd 
\markdownRendererUlItem Messy formatting/absent DOIs → deduct Dim3.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only per schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/f503e83a3debae2296807e472f914b48.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}You are the \markdownRendererStrongEmphasis{Numerical Experiments Reviewer}.\markdownRendererParagraphSeparator
{}Dimension rubric\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Dim1 Sufficiency (25): coverage of typical + edge cases; multiple difficulty levels.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim2 Baseline Fairness (25): fair comparison vs SOTA/classical baselines with matched settings/metrics.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim3 Parameter Specification (15): all key params (grid/step/tol/seeds) stated.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim4 Reproducibility (20): rerun detail—code/links/splits/seeds/ablations.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dim5 Statistical Reliability (15): mean/std over multiple runs when stochastic; variance reported.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Evaluation steps\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}List tasks/datasets/cases; judge diversity and relevance.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Inspect baselines and fairness (same splits, metrics, tuning budgets).\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Collect hyper/solver params; note missing ones.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Check for code/links/seeds/ablations; assess rerun feasibility.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{5}For stochastic settings, verify repeats and variance reporting.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}Scoring rules\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Single easy case or missing baselines → large deduct Dim1/Dim2.\markdownRendererUlItemEnd 
\markdownRendererUlItem Missing key params/seeds → deduct Dim3/Dim4.\markdownRendererUlItemEnd 
\markdownRendererUlItem No repeats in stochastic setting → deduct Dim5 (or 70 “not applicable” if deterministic).\markdownRendererUlItemEnd 
\markdownRendererUlItem Fabricated-looking tables or impossible gains → cap total at 30 pending credibility.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Output\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem JSON only with given schema.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererDocumentEnd

==> _markdown_main/f7cb1ee2e82d7276319c204ba8450240.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererWarning{The `hybrid` option has been soft-deprecated.}{The `hybrid` option has been soft-deprecated.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}{Consider using one of the following better options for mixing TeX and markdown: `contentBlocks`, `rawAttribute`, `texComments`, `texMathDollars`, `texMathSingleBackslash`, and `texMathDoubleBackslash`. For more information, see the user manual at <https://witiko.github.io/markdown/>.}Run-time data blocks (inserted at the top of the prompt before the rubric):\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<assets>} ... full research materials for the paper under evaluation ... \markdownRendererCodeSpan{</assets>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<reference\markdownRendererUnderscore{}signals>} ... programmatic anchor signals from the source assets ... \markdownRendererCodeSpan{</reference\markdownRendererUnderscore{}signals>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<paper>} ... the manuscript produced by the system under review ... \markdownRendererCodeSpan{</paper>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<cite\markdownRendererUnderscore{}check>} ... citation-set operations between source and paper ... \markdownRendererCodeSpan{</cite\markdownRendererUnderscore{}check>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererSoftLineBreak
{}\markdownRendererCodeSpan{<paper\markdownRendererUnderscore{}signals>} ... figures used by the paper, figures present in assets but unused, and section-heading structure ... \markdownRendererCodeSpan{</paper\markdownRendererUnderscore{}signals>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<task>} You are the Asset Usage Judgment Reviewer. Given the input assets and the generated paper, judge whether the paper made reasonable editorial choices about which materials to include. Reasonable usage requires two things simultaneously: on the positive side, the core content of the source assets must be represented in the paper; on the negative side, the paper must not indiscriminately include non-core, redundant, or debug material as if it were important content. Your output is a strict JSON report with integer scores from 0 to 10 on five sub-dimensions plus a list of findings. Do not judge content correctness (Phase 1), writing style (Phase 3), or compilation and layout (Phase 4). \markdownRendererCodeSpan{</task>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<rubric>} The five sub-dimensions each weigh the missing-core side and the junk-inclusion side independently. II1 Theorem Usage asks whether the core theorems (those declared core in \markdownRendererCodeSpan{<reference\markdownRendererUnderscore{}signals>}) are actually presented and whether technical lemmas are kept out of the main text rather than dumped wholesale. II2 Algorithm Usage asks whether the problem definition, assumptions, and pseudocode are all present and whether design-rationale drafts are rewritten into the method discussion rather than pasted verbatim. II3 Experiment Usage asks whether every standalone experiment section from the source is represented in the paper, whether raw data tables are accompanied by analysis rather than stacked into an appendix, and whether no experiment sections appear that are not present in the source. II4 Figure Usage asks whether the core figures identified via \markdownRendererCodeSpan{<paper\markdownRendererUnderscore{}signals>} are used and whether debug or intermediate figures have been kept out of the main text. II5 Citation Usage asks whether foundational references for the paper's topic are cited (reviewers identify these from training knowledge; the rubric itself never names any specific paper) and whether the overall citation count is reasonable. Each sub-dimension is scored on the same 0-10 scale: 10 when the core is fully covered and no junk has accumulated; 8 or 9 for one minor omission or a couple of pieces of junk with the core still intact; 6 or 7 for one core omission or three or more junk pieces; 4 or 5 for multiple core omissions or large-scale junk; 2 or 3 for both widespread missing core and large-scale junk; 0 or 1 when there is almost no reasonable editorial judgment. \markdownRendererCodeSpan{</rubric>}\markdownRendererInlineHtmlTag{<br>}\markdownRendererParagraphSeparator
{}\markdownRendererCodeSpan{<output\markdownRendererUnderscore{}schema>} Return JSON only with per-sub-dimension integer scores and findings. The rubric itself must not name any specific paper, method, or reference; reviewers identify landmarks from their own training knowledge. \markdownRendererCodeSpan{</output\markdownRendererUnderscore{}schema>}\markdownRendererDocumentEnd

==> _markdown_main/frozenCache.tex <==
\expandafter\global\expandafter\def\csname markdownFrozenCache0\endcsname{\input{./_markdown_main/5824be34c5d9c2a53ac24c8c3ad6b93d.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache1\endcsname{\input{./_markdown_main/b791545c349e3fb3beeae6de1fc617d6.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache2\endcsname{\input{./_markdown_main/f503e83a3debae2296807e472f914b48.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache3\endcsname{\input{./_markdown_main/59fcbf975227938e36d846e43162f70b.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache4\endcsname{\input{./_markdown_main/0d086f3d8e5779ac846b5728abb84b85.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache5\endcsname{\input{./_markdown_main/e1c75fe3e92b3c6427ac68bc54d0bd00.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache6\endcsname{\input{./_markdown_main/64f3061720ec9e618a8e904352a0ccf1.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache7\endcsname{\input{./_markdown_main/64617f16f971aad351ce709a5fd3e8ea.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache8\endcsname{\input{./_markdown_main/0f7040eb571eee872cd1e385f6c68bcf.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache9\endcsname{\input{./_markdown_main/8f4594cf74488b5a395b562b6ffbc965.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache10\endcsname{\input{./_markdown_main/cfe8dabfe6b637e6af48641f720c506c.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache11\endcsname{\input{./_markdown_main/582bcfb60cfdd52e575e2e2096c23f54.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache12\endcsname{\input{./_markdown_main/dedd9dcc1c0d3449d9c47b95325e8166.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache13\endcsname{\input{./_markdown_main/98bc1c539b3b1e9e95b6e00e4029df9e.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache14\endcsname{\input{./_markdown_main/dbf3c7bbf09fb40c807956d7f7cb9ea7.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache15\endcsname{\input{./_markdown_main/c4882964c2c6314d38f342adc56fe344.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache16\endcsname{\input{./_markdown_main/50aa72a1f259250205ef95b9f920b85f.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache17\endcsname{\input{./_markdown_main/32f990fbeb9b78fd455b464fed370efc.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache18\endcsname{\input{./_markdown_main/bb61e96c925293198eed49e7f0d47326.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache19\endcsname{\input{./_markdown_main/298de318060dbfcb082ecaabbfeffdfb.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache20\endcsname{\input{./_markdown_main/d899060c6c71c792f8d69f679aab1df2.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache21\endcsname{\input{./_markdown_main/f7cb1ee2e82d7276319c204ba8450240.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache22\endcsname{\input{./_markdown_main/9f6cf099e407d45ea80ee9e4114d9048.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache23\endcsname{\input{./_markdown_main/d17bd8b3edf2485703d1d52038dc1df6.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache24\endcsname{\input{./_markdown_main/73a5e60091e72134b6262bc8836b816b.md.tex}\relax}

